Development Effort Estimation in Free/Open Source Software from Activity in Version Control Systems

Effort estimation models are a fundamental tool in software management, and used as a forecast for resources, constraints and costs associated to software development. For Free/Open Source Software (FOSS) projects, effort estimation is especially complex: professional developers work alongside occasional, volunteer developers, so the overall effort (in person-months) becomes non-trivial to determine. The objective of this work it to develop a simple effort estimation model for FOSS projects, based on the historic data of developers' effort. The model is fed with direct developer feedback to ensure its accuracy. After extracting the personal development profiles of several thousands of developers from 6 large FOSS projects, we asked them to fill in a questionnaire to determine if they should be considered as full-time developers in the project that they work in. Their feedback was used to fine-tune the value of an effort threshold, above which developers can be considered as full-time. With the help of the over 1,000 questionnaires received, we were able to determine, for every project in our sample, the threshold of commits that separates full-time from non-full-time developers.%, and that minimizes the type I and type II errors. We finally offer guidelines and a tool to apply our model to FOSS projects that use a version control system.

==> 01c-vision.tex <==
\section{Rationale and Application of our Model}
\label{sec:_vision}

The model that we propose is based on an overarching rationale, that is set (1) to minimize the effort estimation error using reasonable assumptions, and (2) to simplify the applicability of our model in other FOSS projects. Thus, the model builds on data that can be extracted from the VCS of a project, and is supported by specific feedback from project developers.

In this section, we offer an overview of the most relevant aspects of the model. 
Details will be elaborated in the rest of the paper.

\subsection{Calculating an upper bound of effort into a project}
\label{subsec:_upper}

If we would like to calculate easily an upper bound of the effort in a project, we could consider all its commiters in a given month to have been working on that project all the time, as if they would have been full-time developers on it. Hence, no matter what the contribution of a developer is, having one commit would add 1 PM (person-month) of effort to the project. Any further commit in that month won't add to the effort as 1PM is the maximum that a developer can have in one month; we refer this effect as \emph{saturation}.

Although this approach is very coarse, it already offers a good starting point to have a first, inaccurate approximation. The major source of error comes from the fact that many contributors are non-full-time developers. This is because in this first approximation, we have assumed de facto that every committer is a full-time developer. Actually, we know from the research literature that FOSS projects usually follow a very skewed distribution where more than 80\% of the effort is performed by 20\% of the developers. In large FOSS projects, and this includes those of hybrid nature, there is relatively small group of full-time developers and a large number of volunteers. In this scenario we have a small number of developers with a high involvement (i.e., many commits) and a large number with a smaller number of contributions (i.e., less commits)..

\subsection{Identifying full-time developers with an activity threshold}

The question then is: can we identify a threshold value (of commit activity) that allows to discriminate between full-time developers and those who aren't? 

We will call this threshold value $\theta$. In this scenario, for full-time developers (i.e., those above $\theta$), the saturation effect will work - they will all devote 1PM every month. And for non-full-time developers (i.e., those below $\theta$), their contribution will be relative to $\theta$. So, if a developer D contributes with 3 commits and $\theta$ is identified as 10, then her effort in that month will be 3/10 PM.

To ascertain if this is possible, we have (1) gathered data from the VCS of several FOSS projects, and (2) asked developers about their status (full-time / part-time / occasional) in the project. With this information, we have tried to obtain $\theta$ (see below in Section~\ref{subsec:_obtaining}).

From the surveys, we have also noted that considering time windows of one month to determine effort in FOSS is not the best period of time.
The reason for this is that a month is a period that is sensitive to developers taking holidays or of projects being in different stages (e.g., the phase of ''feature freeze'' just before a release has different activities and a different activity level as the bug-hunting phase right after a release), etc.
Hence, their activity level (i.e., the number of commits) could easily depend on them.
A better time window is 6 months, as it smooths holidays and goes hand by hand with the release schedule of many FOSS projects\cn.

\subsection{Obtaining the threshold value $\theta$}
\label{subsec:_obtaining}

Once we had data from the survey and the VCS, we used the usual information retrieval measures to identify $\theta$, such as precision and recall. But we noted that our model is based on the summation of all the individual efforts.
In such a situation, a false positive is neutralized (compensated) by a false negative.
In other words, if we know from the survey that developer F if full-time and developer N is non-full-time, but the activity of F is below $\theta$ and of N is above the threshold, we can consider that the miscalculation for F \emph{compensates} the one for N.

As a result, we arrived to a new measure (which we have called \emph{goodness}) that minimizes the error of effort estimation, although it may be that it does not maximize the values of precision and recall. 
In summary, $\theta$ (i.e., the value that minimizes the error in our estimation) is given by the highest value of goodness (see Section~\ref{sec:_on_goodness} for a more in-depth discussion on the concept of goodness).

\subsection{Application of the model}

\begin{figure*}
\begin{center}
  \includegraphics[keepaspectratio=true,width=0.3\textwidth]{img/model-complete.png}
\label{fig:_application}
\caption{Flowchart of our effort estimation model for FOSS projects.}
\end{center}
\end{figure*}

Figure~\ref{fig:_application} offers a flowchart of how our model can be applied to any FOSS project. 
The different steps are as follows (they will be further elaborated in Section~\ref{sec:model}):

\begin{enumerate}
  \item Survey the developers: The survey does not need to be representative of all the community, but of those developers that are highly active.
  \item Determine $\theta$: Look for the highest value of goodness.
  \item Analyze your repository: Merge identities, count commits
  \item Obtain your effort estimation:
  \begin{itemize}
    \item Developers above $\theta$ are assigned 6PM
    \item Developers below $\theta$ are assigned a relative share of the 6PM depending on their number of commits relative to $\theta$
  \end{itemize}
  \item Sum all individual efforts to obtain the total effort
\end{enumerate}

We have developed a tool that, once $\theta$ has been determined, automates the rest of the steps (git2effort\footnote{http://github.com/gregoriorobles/git2effort}).


\subsection{Simplified application}

The application of our model is easy, but we envision that it could be made even easier in the future by removing the need to survey developers.
This is because we have learned that $\theta$ seems to be dependent on several characteristics of a project, basically how easy it is to integrate code into the project (which has to do with its code review and commit squashing practices, see Section~\fixme).

If this is the case, $\theta$ could be estimated from similar projects (i.e., those who show to have similar characteristics as it is done in other effort estimation models such as Intermediate and Detailed COCOMO \cn). 
In such an scenario, the effort estimation can be done automatically with a tool that we have developed (git2effort), which is highlighted as a box in Figure~\ref{fig:_application}.
In this paper, we provide data for 6 FOSS projects, but given the simplicity of our model, we expect to have many more in the near future.


